Improved Space Bounds for Learning with Experts

We give improved tradeoffs between space and regret for the online learning with expert advice problem over $T$ days with $n$ experts. Given a space budget of $n^{\delta}$ for $\delta \in (0,1)$, we provide an algorithm achieving regret $\tilde{O}(n^2 T^{1/(1+\delta)})$, improving upon the regret bound $\tilde{O}(n^2 T^{2/(2+\delta)})$ in the recent work of [PZ23]. The improvement is particularly salient in the regime $\delta \rightarrow 1$ where the regret of our algorithm approaches $\tilde{O}_n(\sqrt{T})$, matching the $T$ dependence in the standard online setting without space restrictions.

==> old.tex <==
% \subsection{Parameters}

% The following setting of parameters and bound on regret is valid for some values of $\delta$ by using $k$ levels of buckets.
% \begin{itemize}
%     \item $\delta > 1 - \frac{2^k}{2^k k - 2^k + 2}$
%     \item $T_0 = n^{\frac{2^k - (1-\delta) \left(2^k k - 2^k + 2\right)}{2^k - 1}}$
%     \item $T_i = n^{(1-\delta)\left(\frac{2^i i - 2^i + 1}{2^{i-1}}\right)} T_0^{\frac{2^{i+1} - 1}{2^i}}$
%     \item $R = n^{k(1-\delta)}T_0 = T^{\frac{2^k + (1-\delta)\left(2^k - (k+2)\right)}{2^{k+1} - k + 2 + \delta(k+1)}}$
% \end{itemize}

\begin{algorithm}[ht!]
\caption{\label{alg:general} \mainalg}
\begin{flushleft}
{\bfseries Input:} Bucket sizes $T_0 \leq T_1 \leq \ldots \leq T_k=T$ with $T_i \equiv 0 \pmod{T_{i-1}}$ for $i \in [k]$, space parameter $m$, decay rate $\eta$ \todo{do we need different rates?}
\begin{algorithmic}[1]
\State Create $k$ buckets $B_0, \ldots, B_{k-1}$ which will each store tuples of the form (expert, arrival time, mistake counter, weight)
% \State Create $k$ dictionaries $D_0, \ldots, D_{k-1}$ mapping experts in the corresponding bucket to a pair of (arrival time, mistake counter)
% \State Create $k$ dictionaries $w_0, \ldots, w_{k-1}$ mapping experts to weights
\State Independently for each bucket, sample $m$ experts without replacement, set their arrival times and mistake counters to $0$, and set their weights to $1$
\State Create array $w$ of $k$ weights initialized to $1$ (multiplicative weights across levels)
% \For{$i \in \{0, \ldots, k-1\}$} \Comment{Initialization}
%     \State $B_i[0:m] \gets$ random sample of $m$ experts
%     % \State $B_i[m:2m] \gets B_i[0:m]$ 
%     % \State $B_i[2m:3m] \gets B_i[0:m]$
%     \State $D_i[e] \gets (0,0)$ for $e \in B_i$
%     \State $w_i[e] \gets 1$ for $e \in B_i$
% \EndFor
% \State $v[i] \gets 1$ for $i \in \{0,\ldots,k-1\}$ \todo{Change to run multiplicative weights between pairs} \\
\For{day $t$ in $\{1,\ldots, T\}$} \Comment{Main loop}
    \If{$t = 1$} \textbf{output} 0 and continue\EndIf
    \State Create array $p$ of size $k$
    \For{$i \in \{0, \ldots, k-1\}$}
        \For{$e \in B_i$}
            % \State $D_i[e][0] \pluseq 1$ \Comment{Update time}
            \If{$(x_e)_{t-1} \neq y_{t-1}$} 
                \State $D_i[e][1] \pluseq 1$ \Comment{Update mistakes}
                \State $w_i[e] \timeseq (1-\eta)$ \Comment{Multiplicative weights update}
            \EndIf
        \EndFor
        \If{$t \equiv 0 \pmod{T_i}$}\
            \State $B_i[m:2m] \gets \evictionalg(B_i, D_i, m)$ \Comment{Update young pool}
            \State $B_i[0:m] \gets $ random sample of $m$ experts not already in $B$ \Comment{Update sample}
            \State $D_i[e] \gets (t,0)$ for $e \in B_i[0:m]$
            \State $w_i[e] \gets 1$ for $e \in B_i$ \Comment{Reset multiplicative weights}
            \If{$t \equiv 0 \pmod{T_{i+1}}$}
                \State $B_{i}[2m:3m] \gets B_i[m:2m]$ \Comment{Update old pool}
                \State $B_{i+1}[3m:4m] \gets B_i[m:2m]$ \Comment{Pass experts to larger block}
            \EndIf
        \EndIf 
        \State $e' \gets $ random $e \in B_i$ picked proportional to weights $w_i$
        \State $p[i] \gets (x_{e'})_t$ \Comment{Prediction of the $i$th level}
    \EndFor
    \State $i' \gets $ random level from $\{0,\ldots, k-1\}$ pick proportional to weights $v$
    \State \textbf{Output} $p[i']$ \Comment{Final prediction}
    \For{$i \in \{0,\ldots, k-1\}$}
        \If{$p[i] \neq y_{t}$}
            $v[i] \timeseq (1 - \eta)$ \Comment{Multiplicative weights update}
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\end{flushleft}
\end{algorithm}
